A Web Application for Experimenting and Validating Remote Measurement of Vital Signs

With a surge in online medical advising remote monitoring of patient vitals is required. This can be facilitated with the Remote Photoplethysmography (rPPG) techniques that compute vital signs from facial videos. It involves processing video frames to obtain skin pixels, extracting the cardiac data from it and applying signal processing filters to extract the Blood Volume Pulse (BVP) signal. Different algorithms are applied to the BVP signal to estimate the various vital signs. We implemented a web application framework to measure a person's Heart Rate (HR), Heart Rate Variability (HRV), Oxygen Saturation (SpO2), Respiration Rate (RR), Blood Pressure (BP), and stress from the face video. The rPPG technique is highly sensitive to illumination and motion variation. The web application guides the users to reduce the noise due to these variations and thereby yield a cleaner BVP signal. The accuracy and robustness of the framework was validated with the help of volunteers.

==> makeglossaries <==
#!/usr/bin/env perl

# File    : makeglossaries
# Author  : Nicola Talbot
# Version : 1.5 (2008/12/26)
# Description: simple Perl script that calls makeindex or xindy.
# Intended for use with "glossaries.sty" (saves having to remember
# all the various switches)

# This file is distributed as part of the glossaries LaTeX package.
# Copyright 2007 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license of (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

# This work consists of the files glossaries.dtx and glossaries.ins 
# and the derived files glossaries.sty, mfirstuc.sty,
# glossary-hypernav.sty, glossary-list.sty, glossary-long.sty,
# glossary-super.sty, glossaries.perl.
# Also makeglossaries and makeglossaries.
#
# History:
# v1.5 (2008-12-26) :
#   * added support for xindy
#   * picks up ordering information from aux file
# v1.4 (2008-05-10) :
#   * added support for filenames with spaces.
# v1.3 (2008-03-08) :
#   * changed first line from /usr/bin/perl -w to /usr/bin/env perl
#     (Thanks to Karl Berry for suggesting this.)
# v1.2 (2008-03-02) :
#   * added support for --help and --version
#   * improved error handling
# v1.1 (2008-02-13) :
#   * added -w and strict
#   * added check to ensure .tex file not passed to makeglossaries
#
# v1.0 (2007-05-10) : Initial release.

use Getopt::Std;
use strict;
use vars qw($opt_q $opt_t $opt_o $opt_s $opt_p $opt_g $opt_c $opt_r
   $opt_l $opt_i $opt_L $opt_n $opt_C);


$Getopt::Std::STANDARD_HELP_VERSION = 1;

my $version="1.5 (2008-12-26)";

# v1.5 added -L <lang> for xindy (but language can be specified in 
# .tex file)
# v1.5 added -n (print the command that would be issued but
# don't actually run the command)
getopts('s:o:t:p:L:C:ilqrcgn');

unless ($#ARGV == 0)
{
   die "makeglossaries: Need exactly one file argument.\nUse `makeglossaries --help' for help.\n";
}

# define known extensions

my %exttype = (
   main => {in=>'glo', out=>'gls', 'log'=>'glg'},
 );

# v1.5 define require languages for xindy

my %language = ();
my %codepage = ();

my $ext = '';
my $name = $ARGV[0];

# modified this to make sure users don't try passing the
# tex file:
if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
{
  $name = substr($ARGV[0],0,length($ARGV[0])-4);

  $ext = substr($ARGV[0],-3,3);

  if (lc($ext) eq 'tex')
  {
     die("Don't pass the tex file to makeglossaries:\n"
        ."either omit the extension to make all the glossaries, "
        ."or specify one of the glossary files, e.g. $name.glo, to "
        ."make just that glossary.\n")
  }
}

my $istfile = "";

# should letter ordering be used? (v1.5 added)

my $letterordering = defined($opt_l);

# check aux file for other glossary types
# and for ist file name

if (open AUXFILE, "$name.aux")
{
   while (<AUXFILE>)
   {
      if (m/\\\@newglossary\s*\{(.*)\}{(.*)}{(.*)}{(.*)}/
        and ($1 ne 'main'))
      {
         $exttype{$1}{'log'} = $2;
         $exttype{$1}{'out'} = $3;
         $exttype{$1}{'in'}  = $4;

         unless ($opt_q)
         {
            print "added glossary type '$1' ($2,$3,$4)\n";
         }
      }

      if (m/\\\@istfilename\s*{([^}]*)}/)
      {
         $istfile = $1;

         # check if double quotes were added to \jobname
         $istfile=~s/^"(.*)"\.ist$/$1.ist/;
      }

      # v1.5 added
      if (m/\\\@xdylanguage\s*{([^}]+)}{([^}]*)}/)
      {
         $language{$1} = $2;
      }

      # v1.5 added
      if (m/\\\@gls\@codepage\s*{([^}]+)}{([^}]*)}/)
      {
         $codepage{$1} = $2;
      }

      # v1.5 added
      # Allow -l switch to override specification in aux file
      unless (defined($opt_l))
      {
         if (m/\\\@glsorder\s*{([^}]+)}/)
         {
            my $ordering = $1;

            if ($ordering eq "word")
            {
               $letterordering = 0;
            }
            elsif ($ordering eq "letter")
            {
               $letterordering = 1;
            }
            else
            {
               print STDERR
                 "WARNING: Unknown ordering '$letterordering'\n",
                 "Assuming word ordering\n";
               $letterordering = 0;
            }
         }
      }
   }

   close AUXFILE;
}
else
{
   print STDERR "Unable to open $name.aux: $!\n";
}

# has the style file been specified?
unless ($istfile)
{
   die "No \\\@istfilename found in '$name.aux'.\n",
       "Did your LaTeX run fail?\n",
       "Did your LaTeX run produce any output?\n";
}

# v1.5 save the general xindy switches

my $xdyopts = '';

unless ($opt_L eq "")
{
  $xdyopts .= " -L $opt_L";
}

# save all the general makeindex switches

my $mkidxopts = '';

if ($opt_i)
{
   $mkidxopts .= " -i";
}

if ($letterordering)
{
   $mkidxopts .= " -l";
   $xdyopts .= " -M ord/letorder";
}

if ($opt_q)
{
   $mkidxopts .= " -q";
   $xdyopts .= " -q";
}

if ($opt_r)
{
   $mkidxopts .= " -r";
}

if ($opt_c)
{
   $mkidxopts .= " -c";
}

if ($opt_g)
{
   $mkidxopts .= " -g";
}

unless ($opt_p eq "")
{
   $mkidxopts .= " -p $opt_p";
}

unless ($opt_s eq "")
{
   $istfile = $opt_s;
}

# Use xindy if style file ends with .xdy otherwise use makeindex

my $usexindy = $istfile=~m/\.xdy\Z/;

if ($ext ne '')
{
   # an extension has been specified, so only process
   # the specified file
   my %thistype = %{$exttype{'main'}}; #default

   my $thislang = "";
   my $thiscodepage = "";

   foreach my $type (keys %exttype)
   {
      if ($exttype{$type}{'in'} eq $ext)
      {
         %thistype = %{$exttype{$type}};

         $thislang = $language{$type};

         $thiscodepage = $codepage{$type};

         last;
      }
   }

   my $outfile;

   if ($opt_o eq "")
   {
      $outfile = "$name.$thistype{out}";
   }
   else
   {
      $outfile = $opt_o;
   }

   my $transcript;

   if ($opt_t eq "")
   {
      $transcript = "$name.$thistype{'log'}";
   }
   else
   {
      $transcript = $opt_t;
   }

   if ($usexindy)
   {
      &xindy("$name.$ext", $outfile, $transcript,$istfile,
        $thislang, $thiscodepage, $xdyopts, $opt_q, $opt_n);
   }
   else
   {
      &makeindex("$name.$ext",$outfile,$transcript,$istfile,
                 $mkidxopts,$opt_q, $opt_n);
   }
}
else
{
   # no file extension specified so process all glossary types

   foreach my $type (keys %exttype)
   {
      my %thistype = %{$exttype{$type}};

      my $inputfile = "$name.$thistype{in}";

      if (-r $inputfile)
      {
         my $outfile;

         if ($opt_o eq "")
         {
            $outfile = "$name.$thistype{out}";
         }
         else
         {
            $outfile = $opt_o;
         }

         my $transcript;

         if ($opt_t eq "")
         {
            $transcript = "$name.$thistype{'log'}";
         }
         else
         {
           $transcript = $opt_t;
         }

         if ($usexindy)
         {
            &xindy($inputfile,$outfile,$transcript,$istfile,
                   $language{$type},$codepage{$type},
                   $xdyopts,$opt_q,$opt_n);
         }
         else
         {
            &makeindex($inputfile,$outfile,$transcript,
                       $istfile,$mkidxopts,$opt_q,$opt_n);
         }
      }
      else
      {
         print STDERR "No read access for '$inputfile': $!\n";
      }
   }
}

sub makeindex{
   my($in,$out,$trans,$ist,$rest,$quiet,$dontexec) = @_;
   my($name,$cmdstr,$buffer,$n,$i,$j);
   my(@stuff,@item);

   $cmdstr = "$rest -s \"$ist\" -t \"$trans\" -o \"$out\" \"$in\"";

   unless ($quiet)
   {
      print "makeindex $cmdstr\n";
   }

   unless ($dontexec)
   {
      open STATUS, "makeindex $cmdstr 2>&1 |"
         or die "Can't fork: $!\n";

      my $status = '';

      while (<STATUS>)
      {
         $status .= $_;
      }

      close STATUS;

      if ($?)
      {
         my $errno = $?;

         if (open LOGFILE, ">>$trans")
         {
            print LOGFILE "\n$status";
            close LOGFILE;
         }
         else
         {
            print STDERR "Unable to open '$trans' $!\n";
         }

         die "Call to makeindex failed (errno=$errno):\n", $status;
      }

      print $status;
   }
}

sub xindy{
   my($in,$out,$trans,$ist,$language,$codepage,$rest,$quiet,
     $dontexec) = @_;
   my($cmdstr, $langparam, $main);
   my($module);

   $module = $ist;
   $module=~s/\.xdy\Z//;

   # map babel names to xindy names
   if ($language eq "frenchb")
   {
      $language = "french";
   }
   elsif ($language=~/^n?germanb?$/)
   {
      $language = "german";
   }
   elsif ($language eq "magyar")
   {
      $language = "hungarian";
   }
   elsif ($language eq "lsorbian")
   {
      $language = "lower-sorbian";
   }
   elsif ($language eq "norsk")
   {
      $language = "norwegian";
   }
   elsif ($language eq "portuges")
   {
      $language = "portuguese";
   }
   elsif ($language eq "russianb")
   {
      $language = "russian";
   }
   elsif ($language eq "slovene")
   {
      $language = "slovenian";
   }
   elsif ($language eq "ukraineb")
   {
      $language = "ukrainian";
   }
   elsif ($language eq "usorbian")
   {
      $language = "upper-sorbian";
   }

   if ($language)
   {
     $langparam = "-L $language";
   }
   else
   {
     $langparam = "";
   }

   # most languages work with xindy's default codepage, but
   # some don't, so if the codepage isn't specific, check
   # the known cases that will generate an error
   # and supply a default. (For all other cases, it's up to the 
   # user to supply a codepage.)

   if ($codepage eq '')
   {
      if ($language eq 'dutch')
      {
         $codepage = "ij-as-ij";
      }
      elsif ($language eq 'german')
      {
         $codepage = "din";
      }
      elsif ($language eq 'gypsy')
      {
         $codepage = "northrussian";
      }
      elsif ($language eq 'hausa')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'klingon')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'latin')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'mongolian')
      {
         $codepage = "cyrillic";
      }
      elsif ($language eq 'slovak')
      {
         $codepage = "small";
      }
      elsif ($language eq 'spanish')
      {
         $codepage = "modern";
      }
      elsif ($language eq 'vietnamese')
      {
         $codepage = "utf";
      }
   }

   my $codepageparam = "";

   if ($codepage)
   {
      $codepageparam = "-C $codepage";
   }

   $main = join(' ',
      "-I xindy",
      "-M \"$module\"",
      "-t \"$trans\"",
      "-o \"$out\"",
      "\"$in\"");

   $cmdstr = join(' ', $rest, $langparam, $codepageparam, $main);

   unless ($quiet)
   {
      print "xindy $cmdstr\n";
   }

   unless ($dontexec)
   {
      open STATUS, "xindy $cmdstr 2>&1 |" or die "Can't fork: $!\n";

      my $status = '';
      my $warnings = "";
      my $retry ="";

      while (<STATUS>)
      {
         $status .= $_;

         $warnings .= $_ if /WARNING:/;
      }

      close STATUS;

      if ($status=~/Cannot locate xindy module for language ([^\s]+) in codepage ([^\s]+)/)
      {
         $cmdstr = join(' ', $rest, $langparam, $main);

         unless ($quiet)
         {
            my $message = "$&\nRetrying using default codepage.\n";

            print STDERR $message;

            $retry .= $message;

            print "xindy $cmdstr\n";
         }

         open STATUS, "xindy $cmdstr 2>&1 |" 
           or die "Can't fork: $!\n";

         $status = '';

         while (<STATUS>)
         {
            $status .= $_;
         }

         close STATUS;
      }

      if ($status=~/Cannot locate xindy module for language ([^\s]+)/
       and $1 ne 'general')
      {
         $cmdstr = join(' ', $rest, "-L general", $main);

         unless ($quiet)
         {
            my $message = "$&\nRetrying with -L general\n";

            print STDERR $message;
            $retry .= $message;

            print "xindy $cmdstr\n";
         }

         open STATUS, "xindy $cmdstr 2>&1 |" 
           or die "Can't fork: $!\n";

         $status = '';

         while (<STATUS>)
         {
            $status .= $_;
         }

         close STATUS;
      }

      if ($?)
      {
         my $errno = $?;

         if (open LOGFILE, ">>$trans")
         {
            print LOGFILE "\n$status";
            close LOGFILE;
         }
         else
         {
            print STDERR "Unable to open '$trans' $!\n";
         }

         if ($language)
         {
            die "Call to xindy failed (errno=$errno):\n", $status;
         }
         else
         {
            # If the language hasn't been set, then it may be
            # because the document doesn't contain
            # \printglossaries/\printglossary or it may be
            # because the user has a customized style file that
            # contains the language settings.

            die "Call to xindy failed (errno=$errno):\n", $status,
             "\n\nNo language detected.",
             "\nHave you remembered to use \\printglossary\n",
             "or \\printglossaries in your document?\n\n";
         }
      }

      print $status;

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n$warnings";

         if ($retry)
         {
            print LOGFILE "\nmakeglossaries messages:\n\n", $retry;
         }

         close LOGFILE;
      }
      else
      {
         print STDERR "Unable to open '$trans' $!\n";
      }

   }
}

sub HELP_MESSAGE{
   print "\nSyntax : makeglossaries [options] <filename>\n\n";
   print "For use with the glossaries package to pass relevant\n";
   print "files to makeindex or xindy\n\n";
   print "<filename>\tBase name of glossary file(s). This should\n";
   print "\t\tbe the name of your main LaTeX document without any\n";
   print "\t\textension.\n";
   print "\n General Options:\n";
   print "-o <gls>\tUse <gls> as the output file.\n";
   print "-q\t\tQuiet mode\n";
   print "-s <sty>\tEmploy <sty> as the style file\n";
   print "-t <log>\tEmploy <log> as the transcript file\n";

   print "\n Xindy Options:\n";
   print "-L <language>\tUse <language>.\n";

   print "\n Makeindex Options:\n";
   print "-c\t\tCompress intermediate blanks\n";
   print "-g\t\tEmploy German word ordering\n";
   print "-l\t\tLetter ordering\n";   
   print "-p <num>\tSet the starting page number to be <num>\n";
   print "-r\t\tDisable implicit page range formation\n";
   print "\nSee makeindex documentation for further details on these ";
   print "options\n";
}

sub VERSION_MESSAGE{
   print "Makeglossaries Version $version\n";
   print "Copyright (C) 2007 Nicola L C Talbot\n";
   print "This material is subject to the LaTeX Project Public License.\n";
}

1;

